FLASH: Fast Neural Architecture Search with Hardware Optimization

Neural architecture search (NAS) is a promising technique to design efficient and high-performance deep neural networks (DNNs). As the performance requirements of ML applications grow continuously, the hardware accelerators start playing a central role in DNN design. This trend makes NAS even more complicated and time-consuming for most real applications. This paper proposes FLASH, a very fast NAS methodology that co-optimizes the DNN accuracy and performance on a real hardware platform. As the main theoretical contribution, we first propose the NN-Degree, an analytical metric to quantify the topological characteristics of DNNs with skip connections (e.g., DenseNets, ResNets, Wide-ResNets, and MobileNets). The newly proposed NN-Degree allows us to do training-free NAS within one second and build an accuracy predictor by training as few as 25 samples out of a vast search space with more than 63 billion configurations. Second, by performing inference on the target hardware, we fine-tune and validate our analytical models to estimate the latency, area, and energy consumption of various DNN architectures while executing standard ML datasets. Third, we construct a hierarchical algorithm based on simplicial homology global optimization (SHGO) to optimize the model-architecture co-design process, while considering the area, latency, and energy consumption of the target hardware. We demonstrate that, compared to the state-of-the-art NAS approaches, our proposed hierarchical SHGO-based algorithm enables more than four orders of magnitude speedup (specifically, the execution time of the proposed algorithm is about 0.1 seconds). Finally, our experimental evaluations show that FLASH is easily transferable to different hardware architectures, thus enabling us to do NAS on a Raspberry Pi-3B processor in less than 3 seconds.

==> acronyms.tex <==
\newacronym{TDP}{TDP}{thermal design power}
\newacronym[longplural={general-purpose processors}]{GPP}{GPP}{general-purpose processor}
\newacronym[longplural={no-operations}]{NOP}{NOP}{no-operation}
\newacronym{ILP}{ILP}{instruction-level parallelism}
\newacronym{VLIW}{VLIW}{very long instruction word}
\newacronym{DVFS}{DVFS}{dynamic voltage and frequency scaling}
\newacronym{DVS}{DVS}{dynamic voltage scaling}
\newacronym{DMR}{DMR}{dual modular redundancy}
\newacronym{HPC}{HPC}{high-performance computing}
\newacronym{DWC}{DWC}{duplication with comparison}
\newacronym{TMR}{TMR}{triple modular redundancy}
\newacronym{ROB}{ROB}{re-order buffer}
\newacronym{DSE}{DSE}{design space exploration}
\newacronym{TSH}{TSH}{tricriteria scheduling heuristics}
\newacronym{PG}{PG}{power gating}
\newacronym{CG}{CG}{clock gating}
\newacronym[longplural={functional units}]{FU}{FU}{functional unit}
\newacronym{PC}{PC}{program counter}
\newacronym{ECC}{ECC}{error correction code}
\newacronym[longplural={basic blocks}]{BB}{BB}{basic block}
\newacronym{BBHT}{BBHT}{basic block history table}
\newacronym{ASIC}{ASIC}{application-specific integrated circuit}
\newacronym{CMOS}{CMOS}{complementary metal-oxide-semiconductor}
\newacronym{ADPCM}{ADPCM}{adaptive differential pulse-code modulation}
\newacronym{DFT}{DFT}{discrete Fourier transform}
\newacronym{AVF}{AVF}{architectural vulnerability factor}
\newacronym{RTL}{RTL}{register-transfer level}
\newacronym{SET}{SET}{single-event transient}
\newacronym{SEU}{SEU}{single-event upset}
\newacronym{SBU}{SBU}{single bit upset}
\newacronym{MBU}{MBU}{multiple bit upset}
\newacronym[longplural={arithmetic logic units}]{ALU}{ALU}{arithmetic logic unit}
\newacronym{MMX}{MMX}{multimedia extension}
\newacronym{LUDCMP}{LUDCMP}{LU decomposition}
\newacronym{EDFP}{EDFP}{energy-delay-failure product}
\newacronym{EDP}{EDP}{energy-delay product}
\newacronym{ISA}{ISA}{instruction set architecture}
\newacronym{TCL}{TCL}{tool command language}
\newacronym{SEE}{SEE}{single-event effect}
\newacronym{DCT}{DCT}{discrete cosine transform} 
\newacronym{TLP}{TLP}{thread-level paralellism}
\newacronym{SRAM}{SRAM}{static random access memory}
\newacronym{FPGA}{FPGA}{field-programmable gate array}
\newacronym{ABFT}{ABFT}{algorithm-based fault tolerance}
\newacronym{TID}{TID}{total ionizing dose}
\newacronym{NMR}{NMR}{N-modular redundancy}
\newacronym{OoO}{OoO}{out-of-order}
\newacronym{VHDL}{VHDL}{VHSIC hardware description language}
\newacronym{DWP}{DWP}{duplicate when possible}
\newacronym{LANSCE}{LANSCE}{Los Alamos Neutron Science Center}
\newacronym{ACE}{ACE}{architecturally correct execution}
\newacronym{PPI}{PPI}{parallel programming interface}
\newacronym{OpenMP}{OpenMP}{open multi processing}
\newacronym{Pthreads}{Pthreads}{POSIX threads}
\newacronym{MPI}{MPI}{message passing interface}
\newacronym{FIFO}{FIFO}{first-in-first-out}
\newacronym{GCC}{GCC}{GNU compiler collection}
\newacronym{RAW}{RAW}{read after write}
\newacronym{MWPUETF}{MWPUETF}{mean work per unit of energy to failure}
\newacronym{MWTF}{MWTF}{mean work to failure}
\newacronym{LUT}{LUT}{look-Up table}
\newacronym{MITF}{MITF}{mean instructions to failure}
\newacronym{NASA}{NASA}{National Aeronautics and Space Administration}
\newacronym{CPU}{CPU}{central processing unit}
\newacronym{CFG}{CFG}{control flow graph}
\newacronym{MCCP}{MCCP}{multiple clustered core processor}
\newacronym{RMT}{RMT}{redundant multithreading}
\newacronym{IPC}{IPC}{instructions per cycle}
\newacronym{PID}{PID}{process ID}
\newacronym{DPM}{DPM}{dynamic power management}
\newacronym{MLP}{MLP}{multi-layer perceptron}
\newacronym{IPS}{IPS}{instructions per second}
\newacronym{NN}{NN}{neural network}
\newacronym{RC}{RC}{reconfiguration controller}
\newacronym{ML}{ML}{machine learning}
\newacronym{IL}{IL}{imitation learning}
\newacronym[longplural={systems-on-chip}]{SoC}{SoC}{system-on-chip}
\newacronym{WiFi-TX}{WiFi-TX}{WiFi transmitter}
\newacronym{WiFi-RX}{WiFi-RX}{WiFi receiver}
\newacronym{Range-Det}{Range-Det}{range detection}
\newacronym{SCT}{SCT}{single carrier transmitter}
\newacronym{SCR}{SCR}{single carrier receiver}
\newacronym{RT}{RT}{real-time}
\newacronym{RL}{RL}{reinforcement learning}
\newacronym{PMU}{PMU}{performance monitoring unit}
\newacronym{DAG}{DAG}{directed acyclic graph}
\newacronym{PAPI}{PAPI}{performance application programming interface}


